Flight Controller Synthesis Via Deep Reinforcement Learning

Traditional control methods are inadequate in many deployment settings involving control of Cyber-Physical Systems (CPS). In such settings, CPS controllers must operate and respond to unpredictable interactions, conditions, or failure modes. Dealing with such unpredictability requires the use of executive and cognitive control functions that allow for planning and reasoning. Motivated by the sport of drone racing, this dissertation addresses these concerns for state-of-the-art flight control by investigating the use of deep neural networks to bring essential elements of higher-level cognition for constructing low level flight controllers. This thesis reports on the development and release of an open source, full solution stack for building neuro-flight controllers. This stack consists of the methodology for constructing a multicopter digital twin for synthesize the flight controller unique to a specific aircraft, a tuning framework for implementing training environments (GymFC), and a firmware for the world's first neural network supported flight controller (Neuroflight). GymFC's novel approach fuses together the digital twinning paradigm for flight control training to provide seamless transfer to hardware. Additionally, this thesis examines alternative reward system functions as well as changes to the software environment to bridge the gap between the simulation and real world deployment environments. Work summarized in this thesis demonstrates that reinforcement learning is able to be leveraged for training neural network controllers capable, not only of maintaining stable flight, but also precision aerobatic maneuvers in real world settings. As such, this work provides a foundation for developing the next generation of flight control systems.

==> 1_Related/nn.tex <==

\section{Artificial Neural Networks for Control}


==> 2_GymFC/bg1.tex <==
In this section we provide a brief overview of quadcopter flight 
dynamics required to understand this work, and an introduction to developing 
flight control systems with RL.   

\subsection{Quadcopter Flight Dynamics}
\label{sec:flightdyn}
A quadcopter is an aircraft with six degrees of freedom (DOF), three
rotational and three translational. With four control inputs (one to
each motor) this results in an under-actuated system that requires an
onboard computer to compute motor signals to provide stable flight. We
indicate with $\omega_i, i \in {1, \dots, M}$ the rotation speed of
each rotor where $M=4$ is the total number of motors for a quadcopter. These 
have a direct impact on the resulting Euler angles
$\phi, \theta, \psi$, \ie roll, pitch, yaw respectively which provide rotation 
in $D=3$ dimensions.  Moreover,
they produce a certain amount of upward thrust, indicated with $f$.

The aerodynamic effect that each $\omega_i$ produces depends upon the
configuration of the motors.  The most popular configuration is
an ``X'' configuration, depicted in Figure~\ref{fig:axis} which has the motors 
mounted in an ``X" formation relative to what is considered the front of the 
aircraft.  This
configuration provides more stability compared to a ``+'' configuration which in 
contrast has its motor configuration rotated an additional $45^{\circ}$ along 
the z-axis. This is due to the differences in torque generated along each axis 
of rotation in respect to the distance of the motor from the axis.  The aerodynamic affect $u$ that 
each rotor speed $\omega_i$ has on
thrust and Euler angles, is given by:
\begin{align}
u_f &= b ( \omega_1^2 + \omega_2^2 + \omega_3^2 + \omega_4^2)\\
u_\phi &= b ( \omega_1^2 + \omega_2^2 - \omega_3^2 - \omega_4^2)\\
u_\theta &= b ( \omega_1^2 - \omega_2^2 + \omega_3^2 - \omega_4^2)\\
u_\psi &= b ( \omega_1^2 - \omega_2^2 - \omega_3^2 + \omega_4^2)
\label{eq:qc_dynamics}
\end{align}
where $u_f, u_\phi, u_\theta, u_\psi$ is the thrust, roll, pitch, and
yaw effect respectively, while $b$ is a thrust factor that captures
propeller geometry and frame characteristics. 
%
%
%
%
%
For further details
about the mathematical models of quadcopter dynamics please refer
to~\cite{bouabdallah2004design}.

\begin{figure}
	\centering

	\begin{subfigure}[b]{0.55\textwidth}
	%trim l b r t
	{\includegraphics[trim=35 405 20 100, clip, width=\textwidth]{fd}}
	\caption{Axis of rotation}
	\label{fig:axis}
	\end{subfigure} \\	
	
	\begin{subfigure}[b]{\textwidth}
		\centering
		\begin{subfigure}[b]{0.25\textwidth}
		%trim l b r t
		{\includegraphics[trim=30 660 470 18, clip, 
		width=\textwidth]{rollright}}
		\caption{Roll right}
		\label{fig:fd:roll}
		\end{subfigure}
        ~
		\begin{subfigure}[b]{0.25\textwidth}
		%trim l b r t
		{\includegraphics[trim=28 660 473 20, clip,
		width=\textwidth]{pitchpos}}
		\caption{Pitch forward}
		\label{fig:fd:pitch}
		\end{subfigure}
        ~
		\begin{subfigure}[b]{0.25\textwidth}
		%trim l b r t
		{\includegraphics[trim=30 660 470 20, clip, width=\textwidth]{yawcw}}
		\caption{Yaw  clockwise}
		\label{fig:fd:yaw}
		\end{subfigure}

	\end{subfigure}
	\caption{Quadcopter rotational movement.}
\label{fig:quadcopter}
\end{figure}

To perform a rotational movement the velocity of each rotor is manipulated 
according to the relationship expressed in Equation~\ref{eq:qc_dynamics} and as illustrated in 
Figure~\ref{fig:fd:roll}, \ref{fig:fd:pitch}, \ref{fig:fd:yaw}.  For example, to 
roll right (Figure~\ref{fig:fd:roll}) more thrust is delivered to motors~3 and~4. 
Yaw (Figure~\ref{fig:fd:yaw}) is not achieved directly through difference in 
thrust generated by the rotor as roll and pitch are, but instead through a
difference in torque in the rotation speed of rotors spinning in opposite directions.  
For example, as shown in Figure~\ref{fig:fd:yaw}, higher rotation speed for rotors~1 and~4 
allow the aircraft to yaw clockwise. Because a net positive torque counter-clockwise causes the 
aircraft to rotate clockwise due to Newton's second law of motion. 

Attitude, in respect to orientation of a quadcopter, can be expressed by its  
angular velocities of each axis $\Omega=[\Omega_\phi, \Omega_\theta, 
\Omega_\psi]$. The objective of attitude control is to compute the required 
motor signals to achieve some desired attitude $\Omega^*$.

In autopilot systems attitude control is executed as an inner control loop  and 
is time-sensitive.  Once the desired attitude is achieved, translational 
movement (in the X, Y, Z direction) is accomplished by applying thrust 
proportional to each motor.

In commercial quadcopter, the vast if not all use PID attitude control. A PID 
controller is a linear feedback controller expressed mathematically as,
\begin{equation}
	u(t) = K_p e(t) + K_i \int_0^t e(\tau) d \tau + K_d \frac{d e(t)}{dt}
\end{equation}
where $K_p, K_i, K_d$ are configurable constant gains and $u(t)$ is the control 
signal. The effect of each term can be thought of as the P term considers the 
current error, the I term considers the history of errors and the D term 
estimates the future error. For attitude control in a quadcopter aircraft there 
is PID control for each roll, pitch and yaw axis. At each cycle in the inner 
loop, each PID sum is computed for each axis and then these values are 
translated into the amount of power to deliver to each motor through a process 
called \textit{mixing}. Mixing uses a table consisting of constants describing 
the geometry of the frame to determine how the axis control signals are summed 
based on the torques that will be generated by the length of each arm~(recall 
differences between ``X" and ``+" frames).  The control signal for each motor  
$y_i$ is loosely defined as,
%
%
\begin{equation}
y_i=f\left( m_{(i,\phi)} u_\phi + m_{(i,\theta)} u_\theta +m_{(i,\psi)} u_\psi 
\right)
\label{eq:mix}
\end{equation} where $m_{(i,\phi)},m_{(i,\theta)},m_{(i,\psi)}$ are the mixer 
values for motor $i$ and $f$ is the throttle coefficient. 




\subsection{Reinforcement Learning}
\label{sec:rl}
\wil{This needs to be generic here and move stuff specific to gymfc to next chapter}
In this work we consider \new{an RL architecture (depicted in 
Figure~\ref{fig:rlenv}) consisting of} a neural network flight controller as an 
agent  interacting with an Iris quadcopter~\cite{iris} in a high fidelity 
physics simulated  environment $\mathcal{E}$, more specifically using the
Gazebo simulator~\cite{koenig2004design}.   


At each discrete time-step $t$, the agent receives an observation $x_t$ from the 
environments  consisting of the angular velocity error of each axis $e = 
\Omega^* - \Omega$ and the angular velocity of each rotor $\omega_i$ which are 
obtained from the quadcopter's  \new{inertial measurement unit (IMU)} and 
electronic speed controller (ESC) sensors respectively. These observations are 
in the continuous observation spaces $x_t \in \mathbb{R}^{(M+D)}$. 
%
Once the observation  is received, the agent executes an action $a_t$ within 
$\mathcal{E}$.  In return the agent receives a single numerical reward $r_t$ 
indicating the performance of this action.  The action is also in a
continuous action space $a_t \in  \mathbb{R}^M$ and corresponds to the four 
control signals \new{$u(t)$ sent to each ESC driving the attached motor {\small 
		\circled{M}}}.  
%
Because the agent is only receiving this sensor data it is unaware of the 
physical environment and the aircraft dynamics and therefore $\mathcal{E}$ is 
only partially observed by the agent. 
%
%
%
%
Motivated by \cite{mnih2013playing} we consider the state to be a sequence of 
the past observations and actions $s_t = x_i, a_i, \dots, a_{t-1}, x_t$.


%
%

The interaction between the agent and $\mathcal{E}$ is formally defined as a 
Markov decision processes~(MDP) where the state transitions are defined as the 
probability of transitioning to state $s'$ given the current state and action 
are $s$ and $a$ respectively, $Pr\{s_{t+1} = s' | s_t = s, a_t = a\}$.  The 
behavior of the agent is defined by its policy $\pi$ which is essentially a 
mapping of what action should be taken for a particular state.  The objective of 
the agent is to maximize the returned reward overtime to develop an optimal 
policy.  We welcome the reader to refer to \cite{sutton1998reinforcement} for 
further details on \new{RL}.

Up until recently control in continuous action space was considered  difficult 
for RL. Significant progress has been made combining the power of neural 
networks with RL. In this work we elected to use  Deep Deterministic Policy 
Gradient~(DDPG) \cite{lillicrap2015continuous} and Trust Region Policy 
Optimization~(TRPO)~\cite{schulman2015trust} due to the recent use of these 
algorithms for quadcopter navigation control~\cite{hwangbo2017control}.  DDPG 
provides improvement to Deep Q-Network~(DQN)~\cite{mnih2013playing}
for the continuous action domain. It employs an actor-critic architecture using 
two neural networks for each actor and critic.  It is also model-free algorithm 
meaning it can learn the policy without having to first generate a model. TRPO 
is similar to natural gradient policy methods however this method guarantees 
monotonic improvements. We additionally include a third algorithm for our 
analysis called  Proximal Policy Optimization~(PPO) \cite{schulman2017proximal}.  
PPO  is known to out perform other state-of-the-art  methods in challenging 
environments. PPO is also a policy gradient method and has similarities to TRPO 
while being easier to implement and tune. 


\begin{figure*}
    \centering
	{\includegraphics[trim=3 400 335 0, clip, 
	width=0.9\textwidth]{gymfc_rl_env}}
	\caption{\new{RL architecture using the \textsc{GymFC} environment 
	for training intelligent attitude flight controllers.}}
	\label{fig:rlenv}
\end{figure*}



==> 2_GymFC/related.tex <==

As the cost of small scale embedded computing platforms dropped, intelligent 
flight control options became realistic and have been actively researched over 
the last decade to design flight control solutions that are able to 
\textit{adapt}, and  also \textit{learn}. \new{The ability to learn is an 
important distinction that differentiates intelligent control from traditional control algorithms. Intelligent control architectures are capable of  
planning for future events such as  system failure, damage and emergencies, 
tasks that would otherwise be difficult or impossible for other control 
algorithms~\cite{krishnakumar2002intelligent}.}
%

%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
Intelligent PID flight control~\cite{fatan2013adaptive} methods have been 
proposed in which PID gains are dynamically updated online providing adaptive 
control as the environment changes. However these solutions still  
inherit disadvantages associated with PID control, such as integral windup,  
need for mixing, and most significantly, they are feedback controllers and 
therefore inherently \textit{reactive}.  On the other hand feedforward control (or 
predictive control) is \textit{proactive}, and allows the controller to output 
control signals before an error occur. For feedforward control, a model of the system must exist.  
Learning-based intelligent control has been proposed to develop models of the 
aircraft for predictive control using artificial neural networks.  

Notable work by Dierks et. al.~\cite{dierks2010output} proposes an intelligent 
flight control system constructed with neural networks to learn the quadcopter 
dynamics, online, to navigate along a specified path. This method allows the 
aircraft to adapt in real-time to external disturbances and unmodeled dynamics.  
Matlab simulations demonstrate that their approach outperforms a PID controller in the 
presence of unknown dynamics, specifically in regards to control effort 
required to track the desired trajectory. Nonetheless the proposed approach does 
requires prior knowledge of the aircraft mass and moments of inertia to estimate 
velocities.  Online learning is an essential component to constructing a 
complete intelligent flight control system. It is fundamental however to develop 
accurate offline models to account for uncertainties encountered during online 
learning~\cite{santoso2017state}.  
%
%
%
%
%
%
%
%
To build offline models, previous work has used supervised learning to train 
intelligent flight control systems using a variety of data sources such as test 
trajectories~\cite{bobtsov2016hybrid}, and PID step responses 
\cite{shepherd2010robust}.
%
The limitation of this approach is that training data may not accurately reflect 
the underlying dynamics. In general, supervised learning on its own is not ideal 
for interactive problems such as control~\cite{sutton1998reinforcement}.
%
%
%

















\new{RL} has been applied to 
autonomous helicopters to learn how to track trajectories~(guidance) 
specifically how to hover in place and perform various maneuvers
~\cite{bagnell2001autonomous,kim2004autonomous,abbeel2007application}.
Abbeel et. al.~\cite{kim2004autonomous} and Ng et.  
al.~\cite{abbeel2007application} demonstrated their trained helicopter's 
capabilities in helicopter competitions requiring the aircraft to perform 
advanced acrobatic  maneuvers. Performance was compared to trained pilots, 
nevertheless it is unknown how their controllers compare to PID control for 
tracking trajectories. 
%
In contrast to our work, we investigate the use and accuracy of using RL for low 
level manipulation of the aircraft actuators to maintain a desired attitude, not 
for guidance control.  Furthermore our goal is to compare controllers taught with 
RL to PID control to determine what applications, if any, would be more 
appropriate. 
%
The first use of RL in  quadcopter control was presented by Waslander et.  
al.~\cite{waslander2005multi} for altitude control. The authors developed a 
model-based RL algorithm to search for an optimal control policy. The controller 
was rewarded for accurate tracking and damping. Their design provided 
significant improvements in stabilization in comparison to linear control 
system.
%
%
%
More recently Hwangbo et. al.~\cite{hwangbo2017control} has used \new{RL} for 
quadcopter control, particularly for navigation control. They developed a novel 
deterministic on-policy learning algorithm that outperformed 
TRPO~\cite{schulman2015trust} and DDPG~\cite{lillicrap2015continuous} in regards 
to training time. Furthermore the authors validated their results in the real 
world, transferring their simulated model to a physical quadcopter.  Path 
tracking turned out to be adequate.  Notably, the authors discovered major 
differences transferring from simulation to the real world.  Known as the 
\textit{reality gap}, transferring from simulation to the real-world has been 
researched extensively as being problematic without taking additional steps to 
increase realism in the simulator~\cite{jakobi1995noise,miglino1995evolving}.

The vast majority of prior work has focused on performance of navigation and 
guidance. There is limited and insufficient data justifying the accuracy and 
precision of neural-network-based intelligent attitude flight control and none 
to our knowledge for controllers trained using RL. Furthermore this work uses 
physics simulations in contrast to mathematical models of the aircraft and 
environments used in aforementioned prior work for increased realism. {\bf The 
goal of this work is to provide a platform for training attitude controllers 
with RL, and to provide performance baselines in regards to attitude controller 
accuracy.}



==> 3_Neuroflight/bg.tex <==
\subsection{Reinforcement learning}
\subsection{Flight Control System Architecture}

PID Mix vs NN based control 

Basic dynamics
how to achieve tranlational movement? rotate then thrust

different levels of control, inner loop and outter loop

\missingfigure{Overview of the architecture of a flight control system I/O}

The control signal output ($y_i$) represents a percentage of the power to be
delivered to motor $i$ in the range $[0,1]$ where 0.0 is no rotation of the
motor and 1.0
is max rotation. 


==> 3_Neuroflight/discuss.tex <==
Pros

Cons

* Loop speed - What is the max sampling? This is some kinda of law
PID has far less arithmetic operations



What is the minimum model we need to generate a FC?


==> 4_Twin/bg.tex <==
Levels of control


==> 4_Twin/sys.tex <==
\subsection{Simulation Challenges}

Existing multicopter models used for the Gazebo simulator consist of a single body
and the propellers. However Gazebo treats the aircraft body as having a uniform
density thus this does not accuratly relect the real aircraft. In a quadcopter
for example, typically the heaviest components are the battery and motors. In
previous models these are all treated the same.

To increase fidelity we model each individual componenet of the aircraft,
defining  their own geometric properties.  


%
An unexpected result of  modelling each individually component were numerical
instabliities during simulation.  


\todo[inline]{wk: perform experiement to measure at what angular velocity this
occurs at. See if we can take the pose of each motor. Fix the aircraft to one
axis. Increase the control
output while recording the pose. Plot over time. }


==> 4_Twin/table_metrics_sim_ppo_gymfc1.5.tex <==
%
%
%

\def\meta{6\xspace}
\def\metb{5\xspace}
\def\metc{16\xspace}
\def\metd{9\xspace}
\def\mete{343\xspace}
\def\metf{270\xspace}
\def\metg{1,050\xspace}
\def\meth{554\xspace}
\def\meti{6,659\xspace}
\def\metj{5,379\xspace}
\def\metk{16,151\xspace}
\def\metl{9,396\xspace}
\def\metm{343,218\xspace}
\def\metn{270,549\xspace}
\def\meto{1,051,181\xspace}
\def\metp{554,983\xspace}
\def\metq{11,728\xspace}
\def\metr{9,809\xspace}
\def\mets{29,633\xspace}
\def\mett{17,057\xspace}
\def\metu{532,501\xspace}
\def\metv{409,072\xspace}
\def\metw{1,525,763\xspace}
\def\metx{822,445\xspace}


\begin{table}[]
    \centering
{\setlength{\tabcolsep}{0.2em}
\def\arraystretch{1.15}%
\begin{tabular}{l|ccc|c|}
\cline{2-5}
                             & \multicolumn{4}{c|}{NN Controller (PPO)}                                                \\ \hline
\multicolumn{1}{|l|}{Metric} & Roll ($\phi$) & Pitch($\theta$) & Yaw ($\psi$)  & \cellcolor[HTML]{DAE8FC}Average       \\ \hline
\multicolumn{1}{|l|}{MAE}    & \meta         & \metb           & \metc         & \cellcolor[HTML]{DAE8FC}\metd         \\
\multicolumn{1}{|l|}{MSE}    & \mete      & \metf          & \metg        &
\cellcolor[HTML]{DAE8FC}\meth        \\
\multicolumn{1}{|l|}{IAE}    & \meti     & \metj       & \metk     &
\cellcolor[HTML]{DAE8FC}\metl     \\
\multicolumn{1}{|l|}{ISE}    & \metm  & \metn      & \meto    &
\cellcolor[HTML]{DAE8FC}\metp    \\
\multicolumn{1}{|l|}{ITAE}   
& \metq    & \metr    & \mets    & 
\cellcolor[HTML]{DAE8FC}\mett    \\
\multicolumn{1}{|l|}{ITSE}   & \metu & \metv   & \metw &
\cellcolor[HTML]{DAE8FC}\metx \\ \hline
\end{tabular}
}
\caption{\new{Simulation validation of  
        performance metrics of NN controller  
 trained with policy using digital twin. 
Metrics are reported for each individual axis, along with the average.
Lower values are better.}}
\label{tab:twin:sim_valid_ppo}
\end{table}





==> 6_CV/extracurricular.tex <==
%
%
%
\cvsection{Extracurricular Activity}


%
%
%
\begin{cventries}

%
  \cventry
    {Core Member} % Affiliation/role
    {B10S (B1t 0n the Security, Underground hacker team)} % Organization/group
    {S.Korea} % Location
    {Nov. 2011 - PRESENT} % Date(s)
    {
      \begin{cvitems} % Description(s) of experience/contributions/knowledge
        \item {Gained expertise in penetration testing areas, especially targeted on web application and software.}
        \item {Participated on a lot of hacking competition and won a good award.}
        \item {Held several hacking competitions non-profit, just for fun.}
      \end{cvitems}
    }

%
  \cventry
    {Member} % Affiliation/role
    {WiseGuys (Hacking \& Security research group)} % Organization/group
    {S.Korea} % Location
    {Jun. 2012 - PRESENT} % Date(s)
    {
      \begin{cvitems} % Description(s) of experience/contributions/knowledge
        \item {Gained expertise in hardware hacking areas from penetration testing on several devices including wireless router, smartphone, CCTV and set-top box.}
        \item {Trained wannabe hacker about hacking technique from basic to advanced and ethics for white hackers by hosting annual Hacking Camp.}
      \end{cvitems}
    }

%
  \cventry
    {Core Member \& President at 2013} % Affiliation/role
    {PoApper (Developers' Network of POSTECH)} % Organization/group
    {Pohang, S.Korea} % Location
    {Jun. 2010 - Jun. 2017} % Date(s)
    {
      \begin{cvitems} % Description(s) of experience/contributions/knowledge
        \item {Reformed the society focusing on software engineering and building network on and off campus.}
        \item {Proposed various marketing and network activities to raise awareness.}
      \end{cvitems}
    }

%
  \cventry
    {Member} % Affiliation/role
    {PLUS (Laboratory for UNIX Security in POSTECH)} % Organization/group
    {Pohang, S.Korea} % Location
    {Sep. 2010 - Oct. 2011} % Date(s)
    {
      \begin{cvitems} % Description(s) of experience/contributions/knowledge
        \item {Gained expertise in hacking \& security areas, especially about internal of operating system based on UNIX and several exploit techniques.}
        \item {Participated on several hacking competition and won a good award.}
        \item {Conducted periodic security checks on overall IT system as a member of POSTECH CERT.}
        \item {Conducted penetration testing commissioned by national agency and corporation.}
      \end{cvitems}
    }

%
  \cventry
    {Member} % Affiliation/role
    {MSSA (Management Strategy Club of POSTECH)} % Organization/group
    {Pohang, S.Korea} % Location
    {Sep. 2013 - Jun. 2017} % Date(s)
    {
      \begin{cvitems} % Description(s) of experience/contributions/knowledge
        \item {Gained knowledge about several business field like Management, Strategy, Financial and marketing from group study.}
        \item {Gained expertise in business strategy areas and inisght for various industry from weekly industry analysis session.}
      \end{cvitems}
    }

%
\end{cventries}


==> 6_CV/honors.tex <==
%
%
%
\cvsection{Honors \& Awards}


%
%
%
\cvsubsection{International}


%
%
%
\begin{cvhonors}

%
  \cvhonor
    {Finalist} % Award
    {DEFCON 26th CTF Hacking Competition World Final} % Event
    {Las Vegas, U.S.A} % Location
    {2018} % Date(s)

%
  \cvhonor
    {Finalist} % Award
    {DEFCON 25th CTF Hacking Competition World Final} % Event
    {Las Vegas, U.S.A} % Location
    {2017} % Date(s)

%
  \cvhonor
    {Finalist} % Award
    {DEFCON 22nd CTF Hacking Competition World Final} % Event
    {Las Vegas, U.S.A} % Location
    {2014} % Date(s)

%
  \cvhonor
    {Finalist} % Award
    {DEFCON 21st CTF Hacking Competition World Final} % Event
    {Las Vegas, U.S.A} % Location
    {2013} % Date(s)

%
  \cvhonor
    {Finalist} % Award
    {DEFCON 19th CTF Hacking Competition World Final} % Event
    {Las Vegas, U.S.A} % Location
    {2011} % Date(s)

%
  \cvhonor
    {6th Place} % Award
    {SECUINSIDE Hacking Competition World Final} % Event
    {Seoul, S.Korea} % Location
    {2012} % Date(s)

%
\end{cvhonors}


%
%
%
\cvsubsection{Domestic}


%
%
%
\begin{cvhonors}

%
  \cvhonor
    {3rd Place} % Award
    {WITHCON Hacking Competition Final} % Event
    {Seoul, S.Korea} % Location
    {2015} % Date(s)

%
  \cvhonor
    {Silver Prize} % Award
    {KISA HDCON Hacking Competition Final} % Event
    {Seoul, S.Korea} % Location
    {2017} % Date(s)

%
  \cvhonor
    {Silver Prize} % Award
    {KISA HDCON Hacking Competition Final} % Event
    {Seoul, S.Korea} % Location
    {2013} % Date(s)

%
  \cvhonor
    {2nd Award} % Award
    {HUST Hacking Festival} % Event
    {S.Korea} % Location
    {2013} % Date(s)

%
  \cvhonor
    {3rd Award} % Award
    {HUST Hacking Festival} % Event
    {S.Korea} % Location
    {2010} % Date(s)

%
  \cvhonor
    {3rd Award} % Award
    {Holyshield 3rd Hacking Festival} % Event
    {S.Korea} % Location
    {2012} % Date(s)

%
  \cvhonor
    {2nd Award} % Award
    {Holyshield 3rd Hacking Festival} % Event
    {S.Korea} % Location
    {2011} % Date(s)

%
  \cvhonor
    {5th Place} % Award
    {PADOCON Hacking Competition Final} % Event
    {Seoul, S.Korea} % Location
    {2011} % Date(s)

%
\end{cvhonors}


==> 6_CV/interests.tex <==

\cvsection{Interests}

\descriptionstyle{Drone
Racing~~|~~Machine Learning~~|~~Engineering~~|~~Backpacking~~|~~Camping~~|~~Cooking~~|~~Snowboarding~~|~~Surfing~~|~~Music}


==> 6_CV/presentation.tex <==
%
%
%
\cvsection{Presentation}


%
%
%
\begin{cventries}

%
  \cventry
    {Presenter for <Hosting Web Application for Free utilizing GitHub, Netlify and CloudFlare>} % Role
    {DevFest Seoul by Google Developer Group Korea} % Event
    {Seoul, S.Korea} % Location
    {Nov. 2017} % Date(s)
    {
      \begin{cvitems} % Description(s)
        \item {Introduced the history of web technology and the JAM stack which is for the modern web application development.}
        \item {Introduced how to freely host the web application with high performance utilizing global CDN services.}
      \end{cvitems}
    }

%
  \cventry
    {Presenter for <DEFCON 20th : The way to go to Las Vegas>} % Role
    {6th CodeEngn (Reverse Engineering Conference)} % Event
    {Seoul, S.Korea} % Location
    {Jul. 2012} % Date(s)
    {
      \begin{cvitems} % Description(s)
        \item {Introduced CTF(Capture the Flag) hacking competition and advanced techniques and strategy for CTF}
      \end{cvitems}
    }

%
  \cventry
    {Presenter for <Metasploit 101>} % Role
    {6th Hacking Camp - S.Korea} % Event
    {S.Korea} % Location
    {Sep. 2012} % Date(s)
    {
      \begin{cvitems} % Description(s)
        \item {Introduced basic procedure for penetration testing and how to use Metasploit}
      \end{cvitems}
    }

%
\end{cventries}


==> 6_CV/skills.tex <==
%
%
%
\cvsection{Skills}


%
%
%
\begin{cvskills}


%
  \cvskill
    {Webdev} % Category
    {HTML, CSS, JavaScript, Bootstrap, JQuery, Django, Flask} % Skills
  \cvskill
    {Programming} % Category
    {Python, Java, C/C++, Go} % Skills
  \cvskill
    {UAV Building} % Category
    {Soldering, CAD Modeling, 3D Printing} % Skills
  \cvskill
    {ML Tools} % Category
    {Tensorflow, OpenAI Gym/Baselines, Tensorforce} % Skills

%
\end{cvskills}


==> 6_CV/writing.tex <==
%
%
%
\cvsection{Writing}


%
%
%
\begin{cventries}

%
  \cventry
    {Founder \& Writer} % Role
    {A Guide for Developers in Start-up} % Title
    {Facebook Page} % Location
    {Jan. 2015 - PRESENT} % Date(s)
    {
      \begin{cvitems} % Description(s)
        \item {Drafted daily news for developers in Korea about IT technologies, issues about start-up.}
      \end{cvitems}
    }

%
  \cventry
    {Undergraduate Student Reporter} % Role
    {AhnLab} % Title
    {S.Korea} % Location
    {Oct. 2012 - Jul. 2013} % Date(s)
    {
      \begin{cvitems} % Description(s)
        \item {Drafted reports about IT trends and Security issues on AhnLab Company magazine.}
      \end{cvitems}
    }

%
\end{cventries}

